Different Tunes Played with Equal Skill: Exploring a Unified Optimization Subspace for Delta Tuning

Delta tuning (DET, also known as parameter-efficient tuning) is deemed as the new paradigm for using pre-trained language models (PLMs). Up to now, various DETs with distinct design elements have been proposed, achieving performance on par with fine-tuning. However, the mechanisms behind the above success are still under-explored, especially the connections among various DETs. To fathom the mystery, we hypothesize that the adaptations of different DETs could all be reparameterized as low-dimensional optimizations in a unified optimization subspace, which could be found by jointly decomposing independent solutions of different DETs. Then we explore the connections among different DETs by conducting optimization within the subspace. In experiments, we find that, for a certain DET, conducting optimization simply in the subspace could achieve comparable performance to its original space, and the found solution in the subspace could be transferred to another DET and achieve non-trivial performance. We also visualize the performance landscape of the subspace and find that there exists a substantial region where different DETs all perform well. Finally, we extend our analysis and show the strong connections between fine-tuning and DETs.

==> tables/all_tasks.tex <==
\begin{table*}[!ht]
  \centering
  \small
  \caption{The tasks involved in our multi-task setting.}
    \begin{tabular}{clll}
    \toprule
    \textbf{Ontology} & \textbf{Task Name} & \textbf{Reference}\\
    \midrule
    \multirow{6}[2]{*}{cls/sentiment analysis} 
          & amazon review & \citealt{mcauley2013hidden} \\
          & financial\_phrasebank & \citealt{malo2014good} \\
          & glue-sst2 & \citealt{socher-etal-2013-recursive} \\
          & imdb  & \citealt{maas-etal-2011-learning}   \\
          & \textbf{rotten\_tomatoes} & \citealt{pang-lee-2005-seeing} \\
          & \textbf{yelp\_polarity} & \citealt{zhang2015character} \\
    \midrule
    \multirow{3}[2]{*}{cls/emotion} 
          & emotion &	\citealt{saravia-etal-2018-carer} \\
          & tweet\_eval-offensive &	\citealt{barbieri-etal-2020-tweeteval} \\
          & tweet\_eval-stance\_climate &	\citealt{barbieri-etal-2020-tweeteval} \\
          
    \midrule
    \multirow{4}[2]{*}{cls/hate speech detection} 
          &   ethos-directed\_vs\_generalized   &	\citealt{Mollas2020ETHOSAO} \\
          &   ethos-race   &	\citealt{Mollas2020ETHOSAO} \\
          &   \textbf{ethos-gender}   &	\citealt{Mollas2020ETHOSAO} \\
          &   hatexplain &	\citealt{mathew2020hatexplain}  \\
    \midrule
    \multirow{4}[2]{*}{cls/NLI} 
          &  glue-mnli & \citealt{williams-etal-2018-broad}   \\
          &  glue-qnli &	\citealt{rajpurkar-etal-2016-squad}   \\
          &  glue-wnli &	\citealt{faruqui-das-2018-identifying}   \\
          &  superglue-rte & \begin{tabular}[c]{@{}l@{}}\citealt{dagan2005pascal, bar2006second}\\\citealt{giampiccolo2007third, bentivogli2009fifth}\end{tabular}   \\
    \midrule
    \multirow{2}[2]{*}{cls/fact checking} 
          &   health\_fact &	\citealt{kotonya-toni-2020-explainable-automated}  \\
          &   liar  &	\citealt{wang-2017-liar} \\
    \midrule
    \multirow{3}[2]{*}{cls/paraphrase} 
          &   glue-qqp & \href{https://quoradata.quora.com/First-Quora-Dataset-Release-Question-Pairs}{(link)}  \\
          &  medical\_questions\_pairs & \citealt{medical-qqp}  \\
          &  paws & \citealt{zhang-etal-2019-paws}   \\
    \midrule
    \multirow{8}[2]{*}{cls/other} 
          &  circa  &	\citealt{louis2020d}   \\
          &  onestop\_english  &	\citealt{vajjala2018onestopenglish}   \\
          &  trec-finegrained  &	\citealt{li-roth-2002-learning}; \citealt{hovy-etal-2001-toward}   \\
          &  wiki\_auto  &	\citealt{jiang-etal-2020-neural}   \\
          &   google\_wellformed\_query &	\citealt{faruqui-das-2018-identifying}  \\
          &   sms\_spam &	\citealt{sms_spam}   \\
          &   superglue-wic  &	\citealt{pilehvar-camacho-collados-2019-wic} \\
          &   \textbf{superglue-wsc} &	\citealt{levesque2012winograd}  \\
    \midrule
    \multirow{4}[2]{*}{qa/closed-book qa} 
          &  lama-google\_re &	\citealt{petroni-etal-2019-language,petroni2020how}   \\
          &  numer\_sense &	\citealt{lin-etal-2020-birds}   \\
          &  search\_qa  &	\citealt{Dunn2017SearchQAAN}  \\
          &  web\_questions  &	\citealt{berant-etal-2013-semantic}  \\
    \midrule
    \multirow{1}[2]{*}{qa/binary} 
          &  boolq &	\citealt{clark-etal-2019-boolq}   \\
    \bottomrule
    \end{tabular}%
  \label{tab:ontology-1}%
\vspace{-2em}
\end{table*}%

\begin{table*}[b]
  \centering
  \small
    \begin{tabular}{clll}
    \toprule
    \textbf{Ontology} & \textbf{Task Name} 
          & \textbf{Reference}\\
    \midrule
    \multirow{14}[2]{*}{qa/multiple-choice qa} 
          &  \textbf{ai2\_arc} &	\citealt{Clark2018ThinkYH}   \\
          
          &  codah  &	\citealt{chen-etal-2019-codah}  \\
          &  commonsense\_qa &	\citealt{talmor-etal-2019-commonsenseqa}   \\
          &  cosmos\_qa  &	\citealt{huang-etal-2019-cosmos}  \\
          &  dream &	\citealt{saha-etal-2018-duorc}   \\
          &  hellaswag &	\citealt{zellers-etal-2019-hellaswag}   \\
          &  \textbf{qasc}  &	\citealt{khot2020qasc}  \\
          &  sciq  &	\citealt{welbl-etal-2017-crowdsourcing}  \\
          &  quail  &	\citealt{Rogers_Kovaleva_Downey_Rumshisky_2020}  \\
          &  quarel &	\citealt{Tafjord_Clark_Gardner_Yih_Sabharwal_2019}   \\
          &  quartz-no\_knowledge &	\citealt{tafjord-etal-2019-quartz}   \\
          &  race-high &	\citealt{lai-etal-2017-race}   \\
          &  superglue-copa  &	\citealt{gordon-etal-2012-semeval}  \\
          &  wino\_grande &	\citealt{Sakaguchi_Le_Bras_Bhagavatula_Choi_2020}   \\
    \midrule
    \multirow{2}[2]{*}{qa/long-form qa} 
          &  \textbf{eli5-asks} & \citealt{fan-etal-2019-eli5}   \\
          &  eli5-eli5  & \citealt{fan-etal-2019-eli5}  \\
    \midrule
    \multirow{3}[2]{*}{qa/MRC} 
          &  hotpot\_qa  &	\citealt{yang-etal-2018-hotpotqa}  \\
          &  quoref &	\citealt{dasigi-etal-2019-quoref}   \\
          &  superglue-record  & \citealt{Zhang2018ReCoRDBT}  \\
    \midrule
    \multirow{2}[2]{*}{cg/summarization} 
          &  multi\_news & \citealt{fabbri-etal-2019-multi}   \\
          &  xsum &	\citealt{narayan-etal-2018-dont}   \\
    \midrule
    \multirow{2}[2]{*}{cg/other} 
          &  spider &	\citealt{yu-etal-2018-spider}   \\
          &  wikisql &	\citealt{zhongSeq2SQL2017}   \\
    \midrule
    % \multirow{5}[2]{*}{other/linguistic phenomenon} 
    %       & blimp-anaphor\_gender\_agreement  & \citealt{warstadt2019blimp}  \\
    %       & blimp-ellipsis\_n\_bar\_1 & \citealt{warstadt2019blimp}   \\
    %       & blimp-irregular\_past\_participle\_adjectives & \citealt{warstadt2019blimp}   \\
    %       & blimp-wh\_questions\_object\_gap & \citealt{warstadt2019blimp}   \\
    %       & blimp-anaphor\_number\_agreement & \citealt{warstadt2019blimp}   \\
    \parbox[c]{2cm}{other/linguistic phenomenon}
    % \parbox[c][2cm][c]{2cm}{other/linguistic phenomenon}
        %   &  \parbox[c]{4cm}{
          & blimp-anaphor\_gender\_agreement  & \citealt{warstadt2019blimp}  \\
          & blimp-ellipsis\_n\_bar\_1 & \citealt{warstadt2019blimp}   \\
          & blimp-irregular\_past\_participle\_adjectives & \citealt{warstadt2019blimp}   \\
          & blimp-wh\_questions\_object\_gap & \citealt{warstadt2019blimp}   \\
          & \textbf{blimp-anaphor\_number\_agreement} & \citealt{warstadt2019blimp}   \\
    \midrule
    \parbox[c]{2cm}{other/generate explanation} 
          %&  \parbox[c]{4cm}{cos\_e}  \\
          & cos\_e & \citealt{rajani-etal-2019-explain}  \\
    \midrule
    \multirow{1}[2]{*}{other/slot\_filling} 
          &  ade\_corpus\_v2-dosage & \citealt{GURULINGAPPA2012885}   \\
    \midrule
    \multirow{4}[2]{*}{other/other} 
          &   acronym\_identification  & \citealt{pouran-ben-veyseh-etal-2020-acronym}  \\
          &  crawl\_domain &	\citealt{zhang-etal-2020-semi}   \\
          &  proto\_qa &	\citealt{boratko-etal-2020-protoqa}   \\
          &  qa\_srl &	\citealt{he-etal-2015-question}   \\
    \bottomrule
    \end{tabular}%
  \label{tab:ontology-2}%
\end{table*}%


==> tables/dataset_category.tex <==
\begin{table}[t]
    \centering
    \scriptsize
    \begin{tabular}{l r}
    \toprule
    \textbf{Category} & \textbf{Task} \\
    \midrule
    TC & WiC, WSC\\
    \midrule
    PD & QQP, MRPC\\
    \midrule
    LF-QA & Eli5-Eli5, Eli5-Askh, Eli5-Asks\\
    \midrule
    MC-QA & DREAM, QuaRTz, CODAH, \\
    & SuperGLUE-COPA\\
    \midrule
    NLI & MNLI, SuperGLUE-RTE, \\
    & SciTail, GLUE-RTE, \\
    \midrule
    SA & Yelp Polarity, Rotten Tomatoes, \\
    & Amazon Review, SST-2\\
    \bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:dastaset-category}
\end{table}

==> tables/datasets_multitask_source_target.tex <==
\begin{table*}[t]
% \endfirsthead
% \endhead
\small
\begin{tabular}{c c c}
\toprule
\textbf{Category} & \textbf{Task Name} & \textbf{Reference}\\
\midrule
\multirow{3}[2]{*}{cls/sentiment analysis} 
      & \textbf{glue-sst2} & \citealt{socher-etal-2013-recursive} \\
      & rotten\_tomatoes & \citealt{pang-lee-2005-seeing} \\
      & amazon review & \citealt{mcauley2013hidden} \\
\midrule
\multirow{3}[2]{*}{cls/NLI} 
      &  \textbf{glue-mnli} & \citealt{williams-etal-2018-broad}   \\
      &  scitail & \citealt{Khot2018SciTaiLAT}  \\
      &  glue-rte & \citealt{dagan2005pascal} \\
\midrule
\multirow{2}[2]{*}{cls/paraphrase} 
      & \textbf{glue-qqp} & \href{http://data.quora.com/First-Quora-Dataset-Release-Question-Pairs}{(link)}  \\
      &  glue-mrpc & \citealt{dolan2005automatically}  \\
\midrule
\multirow{2}[2]{*}{cls/other} 
      &   \textbf{superglue-wic}  &	\citealt{pilehvar-camacho-collados-2019-wic} \\
      &   superglue-wsc &	\citealt{levesque2012winograd}  \\
\midrule
\multirow{4}[2]{*}{qa/multiple-choice qa} 
      &  \textbf{dream} &	\citealt{sun2019dream}   \\
      &  quartz-no\_knowledge &	\citealt{tafjord-etal-2019-quartz}   \\
      &  codah &	\citealt{chen-etal-2019-codah}   \\
      &  superglue-copa &	\citealt{gordon-etal-2012-semeval}   \\
\midrule
\multirow{3}[2]{*}{qa/long-form qa} 
      & \textbf{eli5-askh}   & \citealt{fan-etal-2019-eli5}   \\
      &  eli5-asks & \citealt{fan-etal-2019-eli5}   \\
      &  eli5-eli5  & \citealt{fan-etal-2019-eli5}  \\
\bottomrule
\end{tabular}
\caption{The tasks involved in the multi-task setting. Dataset written in bold of each task are the source datasets we use for subspace approximation to obtain the hyper-networks, while the other datasets of the same task are the target datasets for subspace optimization and subspace solution transfer.} 
\label{tab:datasets-multitask-source-target}%
\end{table*}%

==> tables/datasets_singletask_source_target.tex <==
\begin{table*}[t]
% \endfirsthead
% \endhead
\small
\centering
\begin{tabular}{c c c}
\toprule
\textbf{Category} & \textbf{Task Name} & \textbf{Reference}\\
\midrule
\multirow{3}[2]{*}{cls/sentiment analysis} 
      & \textbf{glue-sst2} & \citealt{socher-etal-2013-recursive} \\
      & rotten\_tomatoes & \citealt{pang-lee-2005-seeing} \\
      & amazon review & \citealt{mcauley2013hidden} \\
\midrule
\multirow{3}[2]{*}{cls/NLI} 
      &  \textbf{glue-mnli} & \citealt{williams-etal-2018-broad}   \\
      &  scitail & \citealt{Khot2018SciTaiLAT}  \\
      &  glue-rte & \citealt{dagan2005pascal} \\
\midrule
\multirow{2}[2]{*}{cls/paraphrase} 
      & \textbf{glue-qqp} & \href{http://data.quora.com/First-Quora-Dataset-Release-Question-Pairs}{(link)}  \\
      &  glue-mrpc & \citealt{dolan2005automatically}  \\
\midrule
\multirow{2}[2]{*}{cls/other} 
      &   \textbf{superglue-wic}  &	\citealt{pilehvar-camacho-collados-2019-wic} \\
      &   superglue-wsc &	\citealt{levesque2012winograd}  \\
\midrule
\multirow{4}[2]{*}{qa/multiple-choice qa} 
      &  \textbf{dream} &	\citealt{sun2019dream}   \\
      &  quartz-no\_knowledge &	\citealt{tafjord-etal-2019-quartz}   \\
      &  codah &	\citealt{chen-etal-2019-codah}   \\
      &  superglue-copa &	\citealt{gordon-etal-2012-semeval}   \\
\midrule
\multirow{3}[2]{*}{qa/long-form qa} 
      & \textbf{eli5-askh}   & \citealt{fan-etal-2019-eli5}   \\
      &  eli5-asks & \citealt{fan-etal-2019-eli5}   \\
      &  eli5-eli5  & \citealt{fan-etal-2019-eli5}  \\
\bottomrule
\end{tabular}
\caption{The tasks involved in the single-task setting. Dataset written in bold of each task are the source datasets we use for subspace approximation to obtain the hyper-networks, while the other datasets of the same task are the target datasets for subspace optimization and subspace solution transfer.} 
\label{tab:datasets-singletask-source-target}%
\end{table*}%

==> tables/dev_multi_task_solution_transfer.tex <==
\begin{table}[t!]
    \centering
    \scriptsize
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{l *{10}{r}}
    \toprule
          $\mathcal{T}_{\text{test}}$ &
          $\mathbf{A} \!\!\rightarrow\!\! \mathbf{L}$ & $\mathbf{A} \!\!\rightarrow\!\! \mathbf{P}$ & $\mathbf{L} \!\!\rightarrow\!\! \mathbf{A}$ & $\mathbf{L} \!\!\rightarrow\!\! \mathbf{P}$ & 
        $\mathbf{P} \!\!\rightarrow\!\! \mathbf{A}$ & 
        $\mathbf{P} \!\!\rightarrow\!\! \mathbf{L}$ & \textbf{Avg.} \\ 
        \midrule
        Rotten Tomatoes& 99.5 & 94.7 & 96.7 & 94.7 & 98.0 & 97.0 & 96.8\\
        Yelp Polarity & 99.4 & 98.5 & 98.3 & 97.2 & 99.4 & 96.7 & 98.3\\
        \midrule
        WSC & 97.4 & 97.4 & 88.0 & 69.1 & 88.0 & 103.7 & 90.6\\
        \midrule
        AI2 ARC & 76.0 & 83.5 & 87.7 & 79.1 & 87.4 & 83.0 & 82.8\\
        QASC & 77.1 & 61.2 & 42.5 & 76.5 & 63.5 & 45.9 & 61.1\\
        QuaRTz & 90.5 & 73.4 & 73.4 & 83.1 & 81.8 & 73.0 & 79.2 \\
        \midrule
        BLiMP-ANA & 100.0 & 91.0 & 51.0 & 100.0 & 100.0 & 49.0 & 81.8\\
        \midrule
        ELI5-Asks & 96.0 & 88.4 & 93.0 & 87.5 & 96.9 & 90.1 & 92.0\\
        \midrule
        ETHOS-Gender & 76.4 & 10.4 & 52.3 & 47.9 & 112.4 & 63.6 & 60.5\\
        \midrule
        \textbf{Avg.} & 90.3 & 77.6 & 75.9 & 81.7 & 91.9 & 78.0 & 82.6 \\
        \bottomrule
    \end{tabular}
    \caption{Relative performance (\%) for subspace solution transfer under the multi-task setting. The solution is selected according to its performance on target \PET.}
    \label{tab:dev-multi-task-solution-transfer}
\end{table}

==> tables/dev_multi_task_subspace_optimization.tex <==
\begin{table}[t!]
    \centering
    \scriptsize
    % \setlength{\tabcolsep}{4pt}
    \begin{tabular}{l *{4}{r}}
    \toprule
        $\mathcal{T}_{\text{test}}$ & \textbf{Adapter} & \textbf{LoRA} & \textbf{Prefix} & \textbf{Avg.} \\
        \midrule
        Rotten Tomatoes & 99.5 & 98.0 & 100.5 & 99.3\\
        Yelp Polarity & 99.4 & 99.4 & 98.9 & 99.2\\
        \midrule
        WSC & 97.4 & 88.0 & 91.1 & 92.2\\
        \midrule
        AI2 ARC & 93.5 & 90.8 & 78.8 & 87.7\\
        QASC & 77.1 & 63.5 & 75.4 & 72.0\\
        QuaRTz & 90.5 & 81.8 & 76.0 & 82.8\\
        \midrule
        BLiMP-ANA & 100.0 & 100.0 & 49.0 & 83.0\\
        \midrule
        ELI5-Asks & 96.0 & 96.9 & 94.3 & 95.7\\
        \midrule
        ETHOS-Gender & 76.4 & 112.4 & 63.6 & 84.1\\
        \midrule
        \textbf{Avg.} & 92.2 & 92.3 & 80.8 & 88.4\\
        \bottomrule
    \end{tabular}
    \caption{Relative performance (\%) for subspace optimization under multi-task setting. The solution is selected according to its performance on target \PET.}
    \label{tab:dev-multi-task-subspace-optimization}
\end{table}

==> tables/dev_single_task_solution_transfer.tex <==
\begin{table}[t!]
    \centering
    \scriptsize
    \setlength{\tabcolsep}{1pt}
    \begin{tabular}{l l *{7}{r}}
    \toprule
        $\mathcal{T}_{\text{train}}$ & $\mathcal{T}_{\text{test}}$ & $\mathbf{A} \!\!\rightarrow\!\! \mathbf{L}$ & $\mathbf{A} \!\!\rightarrow\!\! \mathbf{P}$ & $\mathbf{L} \!\!\rightarrow\!\! \mathbf{A}$ & $\mathbf{L} \!\!\rightarrow\!\! \mathbf{P}$ & 
        $\mathbf{P} \!\!\rightarrow\!\! \mathbf{A}$ & 
        $\mathbf{P} \!\!\rightarrow\!\! \mathbf{L}$ & \textbf{Avg.} \\
        % \cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
        % & & \multicolumn{1}{c}{LoRA} & \multicolumn{1}{c}{Prefix} & \multicolumn{1}{c}{Adapter} & \multicolumn{1}{c}{Prefix} & \multicolumn{1}{c}{Adapter} & \multicolumn{1}{c}{LoRA} & \\
        \midrule
        \multirow{2}{*}{SST-2} & R. Tomatoes & 100.6 & 99.8 & 100.8 & 99.0 & 101.3 & 101.1 & 100.4 \\
        & A. Review & 96.1 & 96.5 & 96.3 & 96.5 & 96.0 & 95.7 & 96.2 \\
        \midrule
        \multirow{2}{*}{MNLI} & SciTail & 82.1 & 77.9 & 80.1 & 81.7 & 81.6 & 79.9 & 80.6 \\
        & RTE & 48.8 & 66.6 & 82.5 & 74.1 & 48.7 & 69.4 & 65.0 \\
        \midrule
        \multirow{1}{*}{WiC} & WSC & 67.6 & 55.9 & 58.8 & 64.7 & 91.2 & 73.5 & 68.6 \\
        \midrule
        \multirow{1}{*}{QQP} & MRPC & 84.8 & 53.4 & 84.8 & 64.0 & 85.4 & 83.1 & 75.9 \\
        \midrule
        \multirow{2}{*}{ELI5-ELI5} & ELI5-Askh & 88.1 & 83.0 & 85.1 & 82.1 & 83.6 & 86.6 & 84.8 \\
        & ELI5-Asks & 97.2 & 92.1 & 86.5 & 88.7 & 95.3 & 96.4 & 92.7 \\
        \midrule
        \multirow{3}{*}{DREAM} & QuaRTz & 54.0 & 72.6 & 70.9 & 73.0 & 74.7 & 77.1 & 70.4 \\
        & CODAH & 63.7 & 66.2 & 65.9 & 23.0 & 79.6 & 71.5 & 61.7 \\
        & CoPA & 76.0 & 109.0 & 105.0 & 70.8 & 88.8 & 65.7 & 85.9 \\
        \midrule
        & \textbf{Avg.} & 78.1 & 79.4 & 83.3 & 74.3 & 84.2 & 81.8 & 80.2\\
        \bottomrule
    \end{tabular}
    \caption{Relative performance (\%) for subspace solution transfer under single-task setting. $\mathbf{A}$, $\mathbf{P}$, and $\mathbf{L}$ refer to Adapter, Prefix-tuning, and LoRA, respectively. The solution is selected according to its performance on target \PET.}
    % R.Tomatoes refers to Rotten Tomatoes, and A. Reivew refers to Amazon Review.}
    \label{tab:dev-single-task-solution-transfer}
\end{table}

==> tables/dev_single_task_subspace_optimization.tex <==
\begin{table}[t!]
    \centering
    \scriptsize
    \setlength{\tabcolsep}{5pt}
    \begin{tabular}{l l *{4}{r}}
    \toprule
        $\mathcal{T}_{\text{train}}$ & $\mathcal{T}_{\text{test}}$ & \textbf{Adapter} & \textbf{LoRA} & \textbf{Prefix} & \textbf{Avg.} \\
        \midrule
        \multirow{2}{*}{SST-2} & Rotten Tomatoes & 101.5 & 100.6 & 99.2 & 100.4 \\
         & Amazon Review & 96.7 & 95.9 & 96.7 & 96.4 \\
        \midrule
        \multirow{2}{*}{MNLI} & SciTail & 83.8 & 80.0 & 82.2 & 82.0 \\
        & RTE & 96.6 & 73.1 & 76.9 & 82.2 \\
        \midrule
        \multirow{1}{*}{WiC} & WSC & 73.5 & 55.9 & 61.8 & 63.7 \\
        \midrule
        \multirow{1}{*}{QQP} & MRPC & 83.7 & 80.9 & 79.2 & 81.3 \\
        \midrule
        \multirow{2}{*}{ELI5-ELI5} & ELI5-Askh & 86.6 & 87.2 & 84.1 & 86.0 \\
        & ELI5-Asks & 95.9 & 95.7 & 94.7 & 95.4 \\
        \midrule
        \multirow{3}{*}{DREAM} & CODAH & 75.2 & 75.6 & 80.3 & 77.0 \\
        & QuaRTz & 75.6 & 77.1 & 76.2 & 76.3 \\
        & CoPA & 109.4 & 76.0 & 88.4 & 91.3 \\
        \midrule
        & \textbf{Avg.} & 89.0 & 81.6 & 83.6 & 84.7\\
        \bottomrule
    \end{tabular}
    \caption{Relative performance (\%) for subspace optimization under single-task setting. The solution is selected according to its performance on target \PET.}
    \label{tab:dev-single-task-subspace-optimization}
\end{table}

==> tables/generalize_finetune.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{l|ccccc}
    \toprule
    \diagbox {ST}{TT} & adapter & lora & prefix & FT  \\
    \hline
    adapter &  101.0 & 97.8 & 98.8 & 83.4 \\
    lora & 100.9 & 98.9 & 98.3 & 93.5 \\
    prefix & 100.0 & 99.8 & 97.9 & 93.0 \\
    FT & 100.1 & 98.3 & 98.1 & 93.1 \\
    \bottomrule
    \end{tabular}
    \caption{The ratios(\%) between transferred performance and the performance of the original target tuning method in rotten tomatoes. ST refers to source tuning method, while TT refers to target tuning method. FT refers to fine-tuning by fastfood.}
    \label{tab:generalize_finetune}
\end{table}


==> tables/multi_task_result.tex <==
\begin{table*}[t!]
    \centering
    \small
    % \setlength{\tabcolsep}{4pt}
    \begin{tabular}{l *{10}{r}}
    \toprule
          \textbf{Source \PET} & \multicolumn{3}{c}{Adapter} & \multicolumn{3}{c}{Prefix} & \multicolumn{3}{c}{Lora} & \multirow{2}{*}{Average} \\
          \cmidrule(r){1-1}\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
        \textbf{Target \PET} & \multicolumn{1}{c}{Adapter} & \multicolumn{1}{c}{Prefix} & \multicolumn{1}{c}{Lora} & \multicolumn{1}{c}{Adapter} & \multicolumn{1}{c}{Prefix} & \multicolumn{1}{c}{Lora} & \multicolumn{1}{c}{Adapter} & \multicolumn{1}{c}{Prefix} & \multicolumn{1}{c}{Lora} \\
        \midrule
        \multicolumn{3}{l}{\textit{Sentiment Analysis (SA)}}\\
        Rotten Tomatoes & 99.5 & 40.2 & 96.5 & 95.1 & 98.0 & 93.2 & 97.1 & 32.2 & 100.5 & 83.6\\
        Yelp Polarity & 99.4 & 98.9 & 94.1 & 98.4 & 99.4 & 96.2 & 98.5 & 95.7 & 98.9 & 97.7\\
        \midrule
        \multicolumn{3}{l}{\textit{Natural Language Inference (NLI)}}\\
        GLUE-RTE & 100.9 & 71.6 & 77.1 & 56.9 & 89.0 & 66.1 & 83.5 & 71.6 & 78.9 & 77.3\\
        \midrule
        \multicolumn{3}{l}{\textit{Text Classification (TC)}}\\
        SuperGLUE-WSC & 97.4 & 97.4 & 97.4 & 59.7 & 88.0 & 103.7 & 75.4 & 91.1 & 91.1 & 89.0\\
        \midrule
        \multicolumn{3}{l}{\textit{Multiple-Choice QA}}\\
        AI2 ARC & 93.5 & 84.1 & 80.2 & 83.0 & 90.8 & 81.9 & 86.6 & 83.8 & 78.8 & 84.7\\
        QASC & 77.1 & 58.4 & 37.4 & 84.4 & 63.5 & 39.7 & 57.2 & 46.5 & 75.4 & 59.9\\
        QuaRTz & 90.5 & 73.4 & 73.4 & 84.8 & 81.8 & 73.0 & 80.9 & 72.8 & 76.0 & 78.5\\
        \midrule
        \multicolumn{3}{l}{\textit{Linguistic Phenomenon (LP)}}\\
        BLiMP-ANA & 100.0 & 0.0 & 51.0 & 96.0 & 100.0 & 47.0 & 69.0 & 91.0 & 49.0 & 67.0\\
        \midrule
        \multicolumn{3}{l}{\textit{Long-Form QA}}\\
        ELI5-Asks & 96.0 & 90.8 & 93.3 & 78.9 & 96.9 & 90.5 & 76.7 & 72.5 & 94.3 & 87.8\\
        \midrule
        \multicolumn{3}{l}{\textit{Hate-Speech Detection (HD)}}\\
        ETHOS-Gender & 76.4 & 56.1 & 0.0 & 64.8 & 112.4 & 31.3 & 65.3 & 27.0 & 63.6 & 55.2\\
        \midrule
        Average & 93.1 & 67.1 & 70.0 & 80.2 & 92.0 & 72.3 & 79.0 & 68.4 & 80.7 & -\\
        \bottomrule
    \end{tabular}
    \caption{The results for multi-task setting. BLiMP-ANA is short for BLiMP Anaphor Number Agreement dataset. We report the ratios(\%) between transferred performance and the performance of fine-tuning. The intrinsic dimension is {\color{red} 0} in this table. }
    \label{tab:multi-task-result}
\end{table*}

==> tables/multitask_train_ontology.tex <==
\begin{table*}[!ht]
  \centering
  \small
  \caption{The train tasks involved in our multi-task setting.}
    \begin{tabular}{clll}
    \toprule
    \textbf{Ontology} & \textbf{Task Name} & \textbf{Reference}\\
    \midrule
    \multirow{4}[2]{*}{Train tasks}
          & amazon review & \citealt{mcauley2013hidden} \\
          & financial\_phrasebank & \citealt{malo2014good} \\
          & glue-sst2 & \citealt{socher-etal-2013-recursive} \\
          & imdb  & \citealt{maas-etal-2011-learning}   \\
          & emotion &	\citealt{saravia-etal-2018-carer} \\
          & tweet\_eval-offensive &	\citealt{barbieri-etal-2020-tweeteval} \\
          & tweet\_eval-stance\_climate &	\citealt{barbieri-etal-2020-tweeteval} \\
          &   ethos-directed\_vs\_generalized   &	\citealt{Mollas2020ETHOSAO} \\
          &   ethos-race   &	\citealt{Mollas2020ETHOSAO} \\
          &   hatexplain &	\citealt{mathew2020hatexplain}  \\
          &  glue-mnli & \citealt{williams-etal-2018-broad}   \\
          &  glue-qnli &	\citealt{rajpurkar-etal-2016-squad}   \\
          &  glue-wnli &	\citealt{faruqui-das-2018-identifying}   \\
          &  superglue-rte & \begin{tabular}[c]{@{}l@{}}\citealt{dagan2005pascal, bar2006second}\\\citealt{giampiccolo2007third, bentivogli2009fifth}\end{tabular}   \\
          &   health\_fact &	\citealt{kotonya-toni-2020-explainable-automated}  \\
          &   liar  &	\citealt{wang-2017-liar} \\
          &   glue-qqp & \href{https://quoradata.quora.com/First-Quora-Dataset-Release-Question-Pairs}{(link)}  \\
          &  medical\_questions\_pairs & \citealt{medical-qqp}  \\
          &  paws & \citealt{zhang-etal-2019-paws}   \\
          &  circa  &	\citealt{louis2020d}   \\
          &  onestop\_english  &	\citealt{vajjala2018onestopenglish}   \\
          &  trec-finegrained  &	\citealt{li-roth-2002-learning}; \citealt{hovy-etal-2001-toward}   \\
          &  wiki\_auto  &	\citealt{jiang-etal-2020-neural}   \\
          &   google\_wellformed\_query &	\citealt{faruqui-das-2018-identifying}  \\
          &   sms\_spam &	\citealt{sms_spam}   \\
          &   superglue-wic  &	\citealt{pilehvar-camacho-collados-2019-wic} \\
          &  lama-google\_re &	\citealt{petroni-etal-2019-language,petroni2020how}   \\
          &  numer\_sense &	\citealt{lin-etal-2020-birds}   \\
          &  search\_qa  &	\citealt{Dunn2017SearchQAAN}  \\
          &  web\_questions  &	\citealt{berant-etal-2013-semantic}  \\
          &  boolq &	\citealt{clark-etal-2019-boolq}   \\
    \midrule
    \multirow{11}[2]{*}{qa/multiple-choice qa} 
          &  codah  &	\citealt{chen-etal-2019-codah}  \\
          &  commonsense\_qa &	\citealt{talmor-etal-2019-commonsenseqa}   \\
          &  cosmos\_qa  &	\citealt{huang-etal-2019-cosmos}  \\
          &  dream &	\citealt{saha-etal-2018-duorc}   \\
          &  hellaswag &	\citealt{zellers-etal-2019-hellaswag}   \\
          &  sciq  &	\citealt{welbl-etal-2017-crowdsourcing}  \\
          &  quail  &	\citealt{Rogers_Kovaleva_Downey_Rumshisky_2020}  \\
          &  quarel &	\citealt{Tafjord_Clark_Gardner_Yih_Sabharwal_2019}   \\
          &  race-high &	\citealt{lai-etal-2017-race}   \\
          &  superglue-copa  &	\citealt{gordon-etal-2012-semeval}  \\
          &  wino\_grande &	\citealt{Sakaguchi_Le_Bras_Bhagavatula_Choi_2020}   \\
    \midrule
    \multirow{1}[2]{*}{qa/long-form qa} 
          &  eli5-eli5  & \citealt{fan-etal-2019-eli5}  \\
    \midrule
    \multirow{3}[2]{*}{qa/MRC} 
          &  hotpot\_qa  &	\citealt{yang-etal-2018-hotpotqa}  \\
          &  quoref &	\citealt{dasigi-etal-2019-quoref}   \\
          &  superglue-record  & \citealt{Zhang2018ReCoRDBT}  \\
    \midrule
    \multirow{2}[2]{*}{cg/summarization} 
          &  multi\_news & \citealt{fabbri-etal-2019-multi}   \\
          &  xsum &	\citealt{narayan-etal-2018-dont}   \\
    \midrule
    \multirow{2}[2]{*}{cg/other} 
          &  spider &	\citealt{yu-etal-2018-spider}   \\
          &  wikisql &	\citealt{zhongSeq2SQL2017}   \\
    \midrule
    % \multirow{5}[2]{*}{other/linguistic phenomenon} 
    %       & blimp-anaphor\_gender\_agreement  & \citealt{warstadt2019blimp}  \\
    %       & blimp-ellipsis\_n\_bar\_1 & \citealt{warstadt2019blimp}   \\
    %       & blimp-irregular\_past\_participle\_adjectives & \citealt{warstadt2019blimp}   \\
    %       & blimp-wh\_questions\_object\_gap & \citealt{warstadt2019blimp}   \\
    %       & blimp-anaphor\_number\_agreement & \citealt{warstadt2019blimp}   \\
    \parbox[c]{2cm}{other/linguistic phenomenon}
    % \parbox[c][2cm][c]{2cm}{other/linguistic phenomenon}
        %   &  \parbox[c]{4cm}{
          & blimp-anaphor\_gender\_agreement  & \citealt{warstadt2019blimp}  \\
          & blimp-ellipsis\_n\_bar\_1 & \citealt{warstadt2019blimp}   \\
          & blimp-irregular\_past\_participle\_adjectives & \citealt{warstadt2019blimp}   \\
          & blimp-wh\_questions\_object\_gap & \citealt{warstadt2019blimp}   \\
    \midrule
    \parbox[c]{2cm}{other/generate explanation} 
          %&  \parbox[c]{4cm}{cos\_e}  \\
          & cos\_e & \citealt{rajani-etal-2019-explain}  \\
    \midrule
    \multirow{1}[2]{*}{other/slot\_filling} 
          &  ade\_corpus\_v2-dosage & \citealt{GURULINGAPPA2012885}   \\
    \midrule
    \multirow{4}[2]{*}{other/other} 
          &   acronym\_identification  & \citealt{pouran-ben-veyseh-etal-2020-acronym}  \\
          &  crawl\_domain &	\citealt{zhang-etal-2020-semi}   \\
          &  proto\_qa &	\citealt{boratko-etal-2020-protoqa}   \\
          &  qa\_srl &	\citealt{he-etal-2015-question}   \\
    
    \midrule
    \multirow{4}[2]{*}{cls/sentiment analysis} 
          & amazon review & \citealt{mcauley2013hidden} \\
          & financial\_phrasebank & \citealt{malo2014good} \\
          & glue-sst2 & \citealt{socher-etal-2013-recursive} \\
          & imdb  & \citealt{maas-etal-2011-learning}   \\
    \midrule
    \multirow{3}[2]{*}{cls/emotion} 
          & emotion &	\citealt{saravia-etal-2018-carer} \\
          & tweet\_eval-offensive &	\citealt{barbieri-etal-2020-tweeteval} \\
          & tweet\_eval-stance\_climate &	\citealt{barbieri-etal-2020-tweeteval} \\
    \midrule
    \multirow{3}[2]{*}{cls/hate speech detection} 
          &   ethos-directed\_vs\_generalized   &	\citealt{Mollas2020ETHOSAO} \\
          &   ethos-race   &	\citealt{Mollas2020ETHOSAO} \\
          &   hatexplain &	\citealt{mathew2020hatexplain}  \\
    \midrule
    \multirow{4}[2]{*}{cls/NLI} 
          &  glue-mnli & \citealt{williams-etal-2018-broad}   \\
          &  glue-qnli &	\citealt{rajpurkar-etal-2016-squad}   \\
          &  glue-wnli &	\citealt{faruqui-das-2018-identifying}   \\
          &  superglue-rte & \begin{tabular}[c]{@{}l@{}}\citealt{dagan2005pascal, bar2006second}\\\citealt{giampiccolo2007third, bentivogli2009fifth}\end{tabular}   \\
    \midrule
    \multirow{2}[2]{*}{cls/fact checking} 
          &   health\_fact &	\citealt{kotonya-toni-2020-explainable-automated}  \\
          &   liar  &	\citealt{wang-2017-liar} \\
    \midrule
    \multirow{3}[2]{*}{cls/paraphrase} 
          &   glue-qqp & \href{https://quoradata.quora.com/First-Quora-Dataset-Release-Question-Pairs}{(link)}  \\
          &  medical\_questions\_pairs & \citealt{medical-qqp}  \\
          &  paws & \citealt{zhang-etal-2019-paws}   \\
    \midrule
    \multirow{7}[2]{*}{cls/other} 
          &  circa  &	\citealt{louis2020d}   \\
          &  onestop\_english  &	\citealt{vajjala2018onestopenglish}   \\
          &  trec-finegrained  &	\citealt{li-roth-2002-learning}; \citealt{hovy-etal-2001-toward}   \\
          &  wiki\_auto  &	\citealt{jiang-etal-2020-neural}   \\
          &   google\_wellformed\_query &	\citealt{faruqui-das-2018-identifying}  \\
          &   sms\_spam &	\citealt{sms_spam}   \\
          &   superglue-wic  &	\citealt{pilehvar-camacho-collados-2019-wic} \\
    \midrule
    \multirow{4}[2]{*}{qa/closed-book qa} 
          &  lama-google\_re &	\citealt{petroni-etal-2019-language,petroni2020how}   \\
          &  numer\_sense &	\citealt{lin-etal-2020-birds}   \\
          &  search\_qa  &	\citealt{Dunn2017SearchQAAN}  \\
          &  web\_questions  &	\citealt{berant-etal-2013-semantic}  \\
    \midrule
    \multirow{1}[2]{*}{qa/binary} 
          &  boolq &	\citealt{clark-etal-2019-boolq}   \\
    \midrule
    \multirow{11}[2]{*}{qa/multiple-choice qa} 
          &  codah  &	\citealt{chen-etal-2019-codah}  \\
          &  commonsense\_qa &	\citealt{talmor-etal-2019-commonsenseqa}   \\
          &  cosmos\_qa  &	\citealt{huang-etal-2019-cosmos}  \\
          &  dream &	\citealt{saha-etal-2018-duorc}   \\
          &  hellaswag &	\citealt{zellers-etal-2019-hellaswag}   \\
          &  sciq  &	\citealt{welbl-etal-2017-crowdsourcing}  \\
          &  quail  &	\citealt{Rogers_Kovaleva_Downey_Rumshisky_2020}  \\
          &  quarel &	\citealt{Tafjord_Clark_Gardner_Yih_Sabharwal_2019}   \\
          &  race-high &	\citealt{lai-etal-2017-race}   \\
          &  superglue-copa  &	\citealt{gordon-etal-2012-semeval}  \\
          &  wino\_grande &	\citealt{Sakaguchi_Le_Bras_Bhagavatula_Choi_2020}   \\
    \midrule
    \multirow{1}[2]{*}{qa/long-form qa} 
          &  eli5-eli5  & \citealt{fan-etal-2019-eli5}  \\
    \midrule
    \multirow{3}[2]{*}{qa/MRC} 
          &  hotpot\_qa  &	\citealt{yang-etal-2018-hotpotqa}  \\
          &  quoref &	\citealt{dasigi-etal-2019-quoref}   \\
          &  superglue-record  & \citealt{Zhang2018ReCoRDBT}  \\
    \midrule
    \multirow{2}[2]{*}{cg/summarization} 
          &  multi\_news & \citealt{fabbri-etal-2019-multi}   \\
          &  xsum &	\citealt{narayan-etal-2018-dont}   \\
    \midrule
    \multirow{2}[2]{*}{cg/other} 
          &  spider &	\citealt{yu-etal-2018-spider}   \\
          &  wikisql &	\citealt{zhongSeq2SQL2017}   \\
    \midrule
    % \multirow{5}[2]{*}{other/linguistic phenomenon} 
    %       & blimp-anaphor\_gender\_agreement  & \citealt{warstadt2019blimp}  \\
    %       & blimp-ellipsis\_n\_bar\_1 & \citealt{warstadt2019blimp}   \\
    %       & blimp-irregular\_past\_participle\_adjectives & \citealt{warstadt2019blimp}   \\
    %       & blimp-wh\_questions\_object\_gap & \citealt{warstadt2019blimp}   \\
    %       & blimp-anaphor\_number\_agreement & \citealt{warstadt2019blimp}   \\
    \parbox[c]{2cm}{other/linguistic phenomenon}
    % \parbox[c][2cm][c]{2cm}{other/linguistic phenomenon}
        %   &  \parbox[c]{4cm}{
          & blimp-anaphor\_gender\_agreement  & \citealt{warstadt2019blimp}  \\
          & blimp-ellipsis\_n\_bar\_1 & \citealt{warstadt2019blimp}   \\
          & blimp-irregular\_past\_participle\_adjectives & \citealt{warstadt2019blimp}   \\
          & blimp-wh\_questions\_object\_gap & \citealt{warstadt2019blimp}   \\
    \midrule
    \parbox[c]{2cm}{other/generate explanation} 
          %&  \parbox[c]{4cm}{cos\_e}  \\
          & cos\_e & \citealt{rajani-etal-2019-explain}  \\
    \midrule
    \multirow{1}[2]{*}{other/slot\_filling} 
          &  ade\_corpus\_v2-dosage & \citealt{GURULINGAPPA2012885}   \\
    \midrule
    \multirow{4}[2]{*}{other/other} 
          &   acronym\_identification  & \citealt{pouran-ben-veyseh-etal-2020-acronym}  \\
          &  crawl\_domain &	\citealt{zhang-etal-2020-semi}   \\
          &  proto\_qa &	\citealt{boratko-etal-2020-protoqa}   \\
          &  qa\_srl &	\citealt{he-etal-2015-question}   \\
    \bottomrule
    \end{tabular}%
  \label{tab:multitask_train_ontology}%
\end{table*}%


==> tables/single_task_results.tex <==
\begin{table*}[t!]
    \centering
    \small
    % \setlength{\tabcolsep}{4pt}
    \begin{tabular}{l *{10}{r}}
    \toprule
          \textbf{Source \PET} & \multicolumn{3}{c}{Adapter} & \multicolumn{3}{c}{Prefix} & \multicolumn{3}{c}{Lora} & \multirow{2}{*}{Average} \\
          \cmidrule(r){1-1}\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
        \textbf{Target \PET} & \multicolumn{1}{c}{Adapter} & \multicolumn{1}{c}{Prefix} & \multicolumn{1}{c}{Lora} & \multicolumn{1}{c}{Adapter} & \multicolumn{1}{c}{Prefix} & \multicolumn{1}{c}{Lora} & \multicolumn{1}{c}{Adapter} & \multicolumn{1}{c}{Prefix} & \multicolumn{1}{c}{Lora} \\
        \midrule
        \multicolumn{3}{l}{\textit{Sentiment Analysis (SA)}}\\
        \textbf{SST-2} & \\
        Rotten Tomatoes & 101.5 & 100.3 & 99.5 & 100.8 & 100.6 & 99.0 & 101.3 & 101.2 & 99.2 & 100.4 \\
        Amazon Review & 96.7 & 96.2 & 96.6 & 84.1 & 95.9 & 96.7 & 96.6 & 95.7 & 96.7 & 95.0 \\
        \midrule
        \multicolumn{3}{l}{\textit{Natural Language Inference (NLI)}}\\
        \textbf{MNLI} &  \\
        SciTail & 83.8 & 81.6 & 77.1 & 81.1 & 80.0 & 81.0 & 74.8 & 79.5 & 82.2 & 80.1 \\
        RTE & 92.9 & 71.8 & 68.1 & 79.1 & 78.2 & 71.8 & 65.3 & 73.6 & 71.8 & 74.7 \\
        \midrule
        \multicolumn{3}{l}{\textit{Text Classification (TC)}}\\
        \textbf{WiC} & \\
        WSC & 73.5 & 70.6 & 55.9 & 58.8 & 55.9 & 55.9 & 91.2 & 82.4 & 61.8 & 67.3 \\
        \midrule
        \multicolumn{3}{l}{\textit{Paraphrase Detection (PD)}}\\
        \textbf{QQP} & \\
        MRPC & 83.7 & 80.3 & 54.5 & 82.0 & 80.9 & 68.5 & 39.3 & 83.7 & 79.2 & 72.5 \\
        \midrule
        \multicolumn{3}{l}{\textit{Long-form QA}}\\
        \textbf{Eli5-Eli5} &  \\
        Eli5-Askh & 86.6 & 88.1 & 83.0 & 84.9 & 87.2 & 82.5 & 84.2 & 87.1 & 84.1 & 85.3 \\
        Eli5-Asks & 95.9 & 96.6 & 94.4 & 86.8 & 95.7 & 90.5 & 95.1 & 96.4 & 94.7 & 94.0 \\
        \midrule
        \multicolumn{3}{l}{\textit{Multiple-choice QA}}\\
        \textbf{DREAM} & \\
        QuaRTz & 75.6 & 54.0 & 72.6 & 70.0 & 77.1 & 67.1 & 73.2 & 74.5 & 76.2 & 71.1 \\
        CODAH & 75.2 & 63.7 & 66.5 & 60.8 & 75.6 & 0.0 & 80.0 & 68.5 & 80.3 & 63.4 \\
        SuperGLUE-CoPA & 109.4 & 73.8 & 103.1 & 106.4 & 76.0 & 0.0 & 91.4 & 64.2 & 88.4 & 79.2 \\
        \midrule
        Average & 89.3 & 76.9 & 77.2 & 81.5 & 81.4 & 65.6 & 74.4 & 82.9 & 82.6 & - \\
        \bottomrule
    \end{tabular}
    \caption{The results for single-task setting. We report the percentage of transferred performance to the fine-tuning performance. The intrinsic dimension is \placeholder in this table. The first dataset written in bold of each task are the datasets we use to approximate the common subspace, while the other datasets within the same category are unseen datasets used in subspace optimization and subspace solution transfer.}
    \label{tab:single-task-result}
\end{table*}

==> tables/stage1_result.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{l l r}
    \toprule
        \textbf{Dataset} & \textbf{Task} & \multicolumn{1}{c}{\textbf{Metric}} \\
    \midrule
        MNLI & NLI & 100.7 \\
        WiC & TC & 84.6 \\
        QQP & PD & 100.6 \\
        SST2 & SA & 98.9 \\
        BLiMP-gender & LP & 99.0 \\
        Eli5-Eli5 & LF-QA & 93.7 \\
        CQA & MC-QA & 93.9 \\
    \bottomrule
    \end{tabular}
    \caption{The ratios(\%) of the average performance of the three shared intrinsic vector's pet to the average performance of the officially implemented pet. }
    \label{tab:stage1-result}
\end{table}

==> tables/stage1_result_alldim.tex <==
\textbf{}\begin{table}[t!]
    \centering
    \small
    \setlength{\tabcolsep}{2.5pt}
    \begin{tabular}{l r r r r r r}
    \toprule
         & \multicolumn{6}{c}{\textbf{Intrinsic Space Dimension}} \\
         \cmidrule{2-7}
        \textbf{Dataset} & \multicolumn{1}{c}{\textbf{1}} & \multicolumn{1}{c}{\textbf{2}} & \multicolumn{1}{c}{\textbf{4}} & \multicolumn{1}{c}{\textbf{8}} & \multicolumn{1}{c}{\textbf{16}} & \multicolumn{1}{c}{\textbf{32}} \\
    \midrule
        MNLI & 100.7 & \textbf{101.5} & 100.9 & 99.9 & 100.7 & 101.0 \\
        WiC & \textbf{91.9} & 88.2 & 88.8 & 86.5 & 84.6 & 83.3 \\
        QQP & 100.6 & 100.7 & 100.7 & \textbf{101.4} & 100.6 & 90.6 \\
        SST2 & 99.2 & 98.1 & \textbf{99.3} & 98.4 & 98.9 & 98.8 \\
        BLiMP-gender & \textbf{99.3} & \textbf{99.3} & 99.0 & 99.0 & 99.0 & \textbf{99.3} \\
        % BoolQ & QA & 97.8 & 98.0 & 98.5 & 98.0 & 91.0 & 90.6 \\
        Eli5-Eli5 & 94.1 & \textbf{94.3} & \textbf{94.3} & 93.1 & 93.7 & 93.3 \\
        CQA & 93.4 & 93.2 & \textbf{95.7} & 95.4 & 93.9 & 94.1 \\
    \bottomrule
    \end{tabular}
    
    \caption{Same as \cref{tab:stage1-result}, except that the results of other dimensions are added.}
    \label{tab:stage1-result-alldim}
\end{table}

==> tables/stage2_result.tex <==
\begin{table*}[t!]
    \centering
    \small
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{l *{9}{r}}
    \toprule
          \textbf{Source \PET} & \multicolumn{3}{c}{Adapter} & \multicolumn{3}{c}{Prefix} & \multicolumn{3}{c}{Lora} \\
          \cmidrule(r){1-1}\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
        \textbf{Target \PET} & \multicolumn{1}{c}{Adapter} & \multicolumn{1}{c}{Prefix} & \multicolumn{1}{c}{Lora} & \multicolumn{1}{c}{Adapter} & \multicolumn{1}{c}{Prefix} & \multicolumn{1}{c}{Lora} & \multicolumn{1}{c}{Adapter} & \multicolumn{1}{c}{Prefix} & \multicolumn{1}{c}{Lora} \\
        \midrule
        \multicolumn{3}{l}{\textit{Sentiment Analysis}}\\
        \textbf{SST2} & 99.8 & 99.5 & 98.5 & 100.0 & 100.0 & 97.8 & 99.3 & 99.8 & 98.5 \\
        Rotten Tomatoes & 99.9 & 100.4 & 100.4 & 99.9 & 100.5 & 99.7 & 99.8 & 100.4 & 100.3 \\
        Yelp Review & 94.1 & 97.6 & 96.2 & 94.0 & 97.6 & 96.0 & 94.3 & 97.4 & 96.7 \\
        Amazon Review & 92.6 & 99.2 & 95.1 & 92.3 & 99.0 & 94.9 & 92.6 & 99.2 & 96.0 \\
        \midrule
        \multicolumn{3}{l}{\textit{Linguistic Phenomenon}}\\
        \textbf{BLiMP-gender} & 99.0 & 100.0 & 99.0 & 99.0 & 100.0 & 99.0 & 99.0 & 100.0 & 99.0 \\
        BLiMP-number & 99.0 & 49.0 & 57.0 & 95.0 & 98.0 & 76.0 & 99.0 & 89.0 & 64.0 \\
        \midrule
        \multicolumn{3}{l}{\textit{Natural Language Inference}}\\
        \textbf{MNLI} & 104.4 & 100.5 & 99.9 & 104.4 & 100.3 & 99.8 & 104.5 & 100.1 & 99.9 \\
        SciTail & 79.9 & 68.6 & 76.5 & 69.9 & 83.0 & 75.2 & 79.3 & 80.6 & 77.9 \\
        RTE & 108.8 & 73.7 & 76.4 & 95.1 & 94.7 & 85.5 & 106.9 & 84.2 & 90.0 \\
        \midrule
        \multicolumn{3}{l}{\textit{Text Classification}}\\
        \textbf{WiC} & 101.4 & 86.7 & 89.0 & 97.6 & 87.1 & 84.5 & 100.0 & 86.7 & 89.0 \\
        WSC & 88.6 & 67.6 & 93.9 & 65.7 & 73.5 & 90.9 & 94.3 & 58.8 & 100.0 \\
        \midrule
        \multicolumn{3}{l}{\textit{Paraphrase Detection}}\\
        \textbf{QQP} & 105.0 & 98.8 & 101.5 & 104.9 & 98.8 & 101.5 & 105.0 & 98.8 & 101.5 \\
        MRPC & 70.2 & 80.3 & 72.5 & 64.0 & 80.3 & 69.1 & 65.7 & 79.8 & 73.0 \\
        \midrule
        \multicolumn{3}{l}{\textit{Long-form QA}}\\
        \textbf{Eli5-Eli5} & 92.5 & 93.9 & 96.8 & 92.9 & 94.1 & 95.3 & 92.4 & 93.9 & 96.4 \\
        Eli5-Askh & 83.9 & 86.6 & 85.2 & 82.7 & 89.3 & 88.0 & 83.9 & 87.3 & 86.3 \\
        Eli5-Asks & 97.7 & 93.7 & 94.1 & 99.4 & 94.1 & 95.0 & 98.1 & 93.6 & 95.3 \\
        \midrule
        \multicolumn{3}{l}{\textit{Multiple-choice QA}}\\
        \textbf{CQA} & 95.5 & 104.0 & 85.6 & 90.2 & 104.3 & 82.7 & 93.8 & 103.8 & 84.8 \\
        QuaRTz & 72.3 & 68.2 & 73.0 & 74.7 & 73.7 & 75.3 & 73.0 & 75.2 & 74.1 \\
        \bottomrule
    \end{tabular}
    \caption{The ratios(\%) between transferred performance and the performance of the target \officialPETs. The intrinsic dimension is 4 in this table. The first row in the title is the source \PET, and the second row in the title is the target \PET. The first dataset written in bold of each task are the datasets we use in stage 1 to obtain the hyper-networks, while the other datasets of the same task are the target datasets of stage 2.}
    \label{tab:stage2-result}
\end{table*}

==> tables/stage2_result_tmp.tex <==
\begin{table*}[t!]
    \centering
    \small
    % \setlength{\tabcolsep}{4pt}
    \begin{tabular}{l l *{9}{r}}
    \toprule
      & &
      \multicolumn{3}{c}{\textbf{Adapter}} & \multicolumn{3}{c}{\textbf{Prefix}} & \multicolumn{3}{c}{\textbf{Lora}} \\
      \cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
     \textbf{Category} & \textbf{Dataset}
     & \multicolumn{1}{c}{\textbf{Adapter}} & \multicolumn{1}{c}{\textbf{Prefix}} & \multicolumn{1}{c}{\textbf{Lora}} & \multicolumn{1}{c}{\textbf{Adapter}} & \multicolumn{1}{c}{\textbf{Prefix}} & \multicolumn{1}{c}{\textbf{Lora}} & \multicolumn{1}{c}{\textbf{Adapter}} & \multicolumn{1}{c}{\textbf{Prefix}} & \multicolumn{1}{c}{\textbf{Lora}} \\
        
    \midrule
    \multirow{4}[2]{*}{SA} &
    \textbf{SST2} & 99.8 & 99.5 & 98.5 & 100.0 & 100.0 & 97.8 & 99.3 & 99.8 & 98.5 \\
    & Rotten Tomatoes & 99.9 & 100.4 & 100.4 & 99.9 & 100.5 & 99.7 & 99.8 & 100.4 & 100.3 \\
    & Yelp Review & 94.1 & 97.6 & 96.2 & 94.0 & 97.6 & 96.0 & 94.3 & 97.4 & 96.7 \\
    & Amazon Review & 92.6 & 99.2 & 95.1 & 92.3 & 99.0 & 94.9 & 92.6 & 99.2 & 96.0 \\
    
    \midrule
    \multirow{2}[2]{*}{LP} & 
    \textbf{BLiMP-gender} & 99.0 & 100.0 & 99.0 & 99.0 & 100.0 & 99.0 & 99.0 & 100.0 & 99.0 \\
    & BLiMP-number & 99.0 & 49.0 & 57.0 & 95.0 & 98.0 & 76.0 & 99.0 & 89.0 & 64.0 \\
    
    \midrule
    \multirow{3}[2]{*}{NLI} & 
    \textbf{MNLI} & 104.4 & 100.5 & 99.9 & 104.4 & 100.3 & 99.8 & 104.5 & 100.1 & 99.9 \\
    & SciTail & 79.9 & 68.6 & 76.5 & 69.9 & 83.0 & 75.2 & 79.3 & 80.6 & 77.9 \\
    & RTE & 108.8 & 73.7 & 76.4 & 95.1 & 94.7 & 85.5 & 106.9 & 84.2 & 90.0 \\
    
    \midrule
    \multirow{2}[2]{*}{TC} & 
    \textbf{WiC} & 101.4 & 86.7 & 89.0 & 97.6 & 87.1 & 84.5 & 100.0 & 86.7 & 89.0 \\
    & WSC & 88.6 & 67.6 & 93.9 & 65.7 & 73.5 & 90.9 & 94.3 & 58.8 & 100.0 \\
    
    \midrule
    \multirow{2}[2]{*}{PD} & 
    \textbf{QQP} & 105.0 & 98.8 & 101.5 & 104.9 & 98.8 & 101.5 & 105.0 & 98.8 & 101.5 \\
    & MRPC & 70.2 & 80.3 & 72.5 & 64.0 & 80.3 & 69.1 & 65.7 & 79.8 & 73.0 \\
    
    \midrule
    \multirow{3}[2]{*}{LF-QA} & 
    \textbf{Eli5-Eli5} & 92.5 & 93.9 & 96.8 & 92.9 & 94.1 & 95.3 & 92.4 & 93.9 & 96.4 \\
    & Eli5-Askh & 83.9 & 86.6 & 85.2 & 82.7 & 89.3 & 88.0 & 83.9 & 87.3 & 86.3 \\
    & Eli5-Asks & 97.7 & 93.7 & 94.1 & 99.4 & 94.1 & 95.0 & 98.1 & 93.6 & 95.3 \\
    
    \midrule
    \multirow{2}[2]{*}{MC-QA} & 
    \textbf{CQA} & 95.5 & 104.0 & 85.6 & 90.2 & 104.3 & 82.7 & 93.8 & 103.8 & 84.8 \\
    & QuaRTz & 72.3 & 68.2 & 73.0 & 74.7 & 73.7 & 75.3 & 73.0 & 75.2 & 74.1 \\
    \bottomrule
    \end{tabular}
    \caption{The ratios(\%) between transferred performance and the performance of the target \officialPETs. The intrinsic dimension is 4 in this table. The first row in the title is the source \PET, and the second row in the title is the target \PET. The first dataset written in bold of each task are the datasets we use in stage 1 to obtain the hyper-networks, while the other datasets of the same task are the target datasets of stage 2.}
    \label{tab:stage2-result-tmp}
\end{table*}
